Probing new physics in the era of precision cosmology

Over the past decades, advancements in observational cosmology have introduced us in an era of precision cosmology, dramatically enhancing our understanding of the Universe's history as well as bringing new tensions to light. Observations of the Cosmic Microwave Background, large-scale structure, and distant galaxies have provided unprecedented insights into the processes that shaped our Universe. This PhD thesis contributes to this research by exploring how these cosmic observables can be leveraged to constrain new physics beyond the standard $\Lambda$-Cold Dark Matter model.

==> Chapters/Notes.tex <==


DIMENSIONS SECTIONS AND TITLES

Conclusion

Read also Reference 8 and table 3 of https://arxiv.org/pdf/1804.01318v1 to put at the beginning


Link the result for nt in the paper 1 with nt in the paper 2

PS is defined $\Delta^2$ so with the square, not without. 

==> Papers/SLCDM/priors.tex <==
\begin{table}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{c@{\hspace{0. cm}}@{\hspace{1.5 cm}} c}
			\hline
			\textbf{Parameter}    & \textbf{Prior} \\
			\hline\hline
			$\Omega_{\rm b} h^2$         & $[0.005\,,\,0.1]$ \\
			$\Omega_{\rm c} h^2$     	 & $[0.001\,,\,0.99]$\\
			$100\,\theta_{\rm {MC}}$     & $[0.5\,,\,10]$ \\
			$\tau$                       & $[0.01\,,\,0.8]$\\
			$\log(10^{10}A_{\rm S})$     & $[1.61\,,\,3.91]$ \\
			$n_{\rm s}$                  & $[0.8\,,\, 1.2]$ \\
			\hline
            $A_0$                        & $[-0.6\,,\,0.6]$\\
            $\epsilon$                 & $[-1\,,0]$\\
            $N_{\rm eff}$                & $[1\,,\,5]$\\
            $m^{\rm eff}_{\nu,\rm sterile}$ [eV]        & $[0\,,\,3]$\\
            $\Sigma m_\nu$ [eV]                & $[0\,,\,2]$\\
            \hline\hline
		\end{tabular}
		\caption{List of the parameter priors. The cutoff for $\epsilon$ is due to the fact that at $\epsilon=0$ we leave the quasi-single-field model and obtain the trispectrum for a multifield inflationary model. 
  }
		\label{tab:Priors}
	\end{center}
\end{table}

==> Papers/SLCDM/table_LCDM.tex <==
\begin{table*}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\resizebox{0.9\textwidth}{!}{\begin{tabular}{c c c c  c  c}
  	        \hline
			\textbf{Parameter} & \textbf{Planck}  & \textbf{Planck+Lensing}  & \textbf{Planck+BAO} & \textbf{Planck+Pantheon} & \textbf{Planck+All} \\
			\hline\hline
			$\Omega_\mathrm{b} h^2$ & $0.02258\pm 0.00017$& $0.02250\pm 0.00016$& $0.02255\pm 0.00015$& $0.02259\pm 0.00017$& $0.02251\pm 0.00014$\\
			$\Omega_\mathrm{c} h^2$ & $0.1185\pm 0.0016$&$0.1187\pm 0.0015$& $0.1187\pm 0.0011$& $0.1183\pm 0.0014$& $0.11861\pm 0.00099$\\
			$100\theta_\mathrm{MC}$ & $1.04110\pm 0.00033$&$1.04105 \pm 0.00033$&$1.04107\pm 0.00029$&$1.04112\pm 0.00032$&$1.04106\pm 0.00029$\\
            $\tau_\mathrm{reio}$ & $0.0516\pm 0.0086$&$0.0512\pm 0.0085$&$0.0514\pm 0.0087$&$0.0515\pm 0.0084$&$0.0510\pm 0.0085$\\
			$\log(10^{10} A_\mathrm{s})$ & $3.160\pm 0.050$&$3.081\pm 0.027$&$3.143\pm 0.043$&$3.162\pm 0.048$&$3.081\pm 0.024$\\
            $n_\mathrm{s}$ & $0.952\pm 0.012$&$0.9586\pm 0.0076$&$0.951\pm 0.011$&$0.952\pm 0.011$&$0.9584\pm 0.0075$\\
			\hline	
            $H_0$ [km s$^{-1}$ Mpc$^{-1}$] & $68.13\pm 0.71$&$67.99\pm 0.68$&$68.01\pm 0.49$&$68.20\pm 0.65$&$68.01\pm 0.45$\\
            $\sigma_8$ & $0.849\pm 0.019$&$0.8190\pm 0.0085$&$0.843\pm 0.016$&$0.849\pm 0.018$&$0.8190^{+0.0084}_{-0.0095}$\\
            $S_8$ & $0.857\pm 0.020$&$ 0.828\pm 0.013$&$ 0.852\pm 0.017$&$ 0.856\pm 0.019$&$ 0.828\pm 0.011$\\
            $A_{\rm 0}$& $-0.116\pm 0.048$&$-0.045\pm 0.029$&$-0.101\pm 0.043$&$-0.118\pm 0.045$&$-0.046^{+0.031}_{-0.027}$\\
            $\epsilon$ &$> -0.369$&$> -0.605$&$> -0.384$&$> -0.325$&$> -0.573$\\
\hline\hline    
		\end{tabular}}
	\end{center}
	\caption{Results for \slcdm. The constraints on parameters are at $68\%$ CL, while upper bounds are at $95\%$ CL.}
	\label{tab:lcdm}
\end{table*}

==> Papers/SLCDM/table_mnu.tex <==
\begin{table*}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\resizebox{0.9\textwidth}{!}{\begin{tabular}{c c c c  c  c}
  	        \hline
			\textbf{Parameter} & \textbf{Planck}  & \textbf{Planck+Lensing}  & \textbf{Planck+BAO} & \textbf{Planck+Pantheon} & \textbf{Planck+All} \\
			\hline\hline
$\Omega_\mathrm{b} h^2 $&$0.02254\pm 0.00018$&$ 0.02245\pm 0.00018$&$ 0.02259\pm 0.00015$&$0.02259\pm 0.00017$&$0.02254\pm 0.00015$\\
$\Omega_\mathrm{c} h^2$&$ 0.1185\pm 0.0015$&$0.1189\pm 0.0015$&$0.1182\pm 0.0013$&$0.1181\pm 0.0015$&$0.1182\pm 0.0012$\\
$100\theta_\mathrm{MC}$&$1.04104\pm 0.00033$&$1.04098\pm 0.00033$&$1.04111\pm 0.00030$&$1.04110\pm 0.00032$&$ 1.04110\pm 0.00030$\\
$\tau$& $0.0509\pm 0.0085$&$0.0507\pm 0.0083$&$0.0518\pm 0.0084$&$ 0.0520\pm 0.0085$&$ 0.0510\pm 0.0086$\\
$\ln(10^{10} A_\mathrm{s})$&$3.183\pm 0.055$&$3.102\pm 0.035$&$3.165\pm 0.052$&$3.177\pm 0.054$&$ 3.096^{+0.034}_{-0.038}$\\
$n_\mathrm{s} $&$0.949\pm 0.012$&$ 0.9555\pm 0.0088$&$0.952\pm 0.012$&$0.952\pm 0.012$&$0.9585\pm 0.0081$\\
\hline
$H_0 $ [km s$^{-1}$ Mpc$^{-1}$] &$66.5^{+2.0}_{-1.7}$&$ 66.4^{+1.7}_{-1.6}$&$67.71\pm 0.61$&$67.6^{+1.2}_{-1.0}$&$67.80\pm 0.57$\\
$\sigma_8$&$0.817^{+0.043}_{-0.036}$&$ 0.789^{+0.033}_{-0.028}$&$ 0.835\pm 0.019$&$0.836\pm 0.027$&$0.812^{+0.015}_{-0.013}$\\
$S_8$& $0.849\pm 0.022$&$ 0.823\pm 0.014$&$ 0.849\pm 0.018$&$ 0.852\pm 0.020$&$ 0.824\pm 0.012$\\
$A_{\rm 0}$&$-0.137\pm 0.051$&$-0.066\pm 0.037$&$-0.120\pm 0.049$&$-0.130\pm 0.051$&$-0.060^{+0.042}_{-0.036}$\\
$\epsilon$&$ > -0.302$&$ > -0.514$&$ > -0.340$&$ > -0.334$&$ > -0.545$\\
$\Sigma m_\nu$ [eV]&$ < 0.624$&$ < 0.542$&$ < 0.266$&$ < 0.356$&$ < 0.236$\\
\hline\hline
            
		\end{tabular}}
	\end{center}
	\caption{Results for \slcdm+$\Sigma m_\nu$. The constraints on parameters are at $68\%$ CL, while upper bounds are at $95\%$ CL.}
	\label{tab:mnu}
\end{table*}

==> Papers/SLCDM/table_mnu_neff.tex <==
\begin{table*}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\resizebox{0.9\textwidth}{!}{\begin{tabular}{c c c c  c  c}
  	        \hline
			\textbf{Parameter} & \textbf{Planck}  & \textbf{Planck+Lensing}  & \textbf{Planck+BAO} & \textbf{Planck+Pantheon} & \textbf{Planck+All} \\
			\hline\hline
$\Omega_\mathrm{b} h^2$ &$0.02245\pm 0.00027$&$0.02230\pm 0.00025$&$0.02252\pm 0.00021$&$0.02255\pm 0.00024$&$ 0.02245\pm 0.00020$\\
$\Omega_\mathrm{c} h^2 $&$ 0.1171\pm 0.0031$&$0.1167\pm 0.0031$&$0.1170\pm 0.0031$&$0.1173\pm 0.0032$&$0.1166\pm 0.0030$\\
$100\theta_\mathrm{MC}$&$1.04121\pm 0.00047$&$1.04125\pm 0.00047$&$1.04128\pm 0.00046$&$1.04122\pm 0.00047$&$1.04131\pm 0.00046$\\
$\tau$&$ 0.0504\pm 0.0088$&$0.0503\pm 0.0083$&$0.0517\pm 0.0086$&$0.0513\pm 0.0086$&$0.0510\pm 0.0086$\\
$\ln(10^{10} A_\mathrm{s})$&$3.173^{+0.061}_{-0.070}$&$3.087^{+0.034}_{-0.039}$&$3.157\pm 0.049$&$3.175\pm 0.060$&$ 3.088^{+0.032}_{-0.038}$\\
$n_\mathrm{s}$&$0.943\pm 0.017$&$0.947\pm 0.013$&$0.946\pm 0.015$&$0.948\pm 0.016$&$0.953\pm 0.011$\\
\hline
$H_0$ [km s$^{-1}$ Mpc$^{-1}$] &$ 65.8\pm 2.2$&$65.3\pm 2.0$&$ 67.3\pm 1.2$&$67.2\pm 1.7$&$67.2\pm 1.1$\\
$\sigma_8$&$0.811^{+0.043}_{-0.038}$&$0.783^{+0.031}_{-0.027}$&$ 0.833\pm 0.019$&$0.834\pm 0.027$&$0.809\pm 0.014$\\
$S_8$ &$0.848\pm 0.022$&$ 0.822\pm 0.014$&$ 0.848\pm 0.018$&$ 0.852\pm 0.021$&$ 0.822\pm 0.012$\\
$A_{\rm 0}$&$-0.133\pm 0.056$&$ -0.058^{+0.038}_{-0.033}$&$-0.116\pm 0.044$&$-0.132\pm 0.052$&$-0.057^{+0.039}_{-0.032}$\\
$\epsilon$&$ > -0.367$&$> -0.591$&$ > -0.355$&$> -0.342$&$ > -0.587$\\
$N_{\rm eff} $&$2.94\pm0.22$&$ 2.88\pm 0.20$&$ 2.96\pm0.19$&$2.99\pm 0.21$&$2.94\pm0.19$\\
$\Sigma m_\nu$ [eV]&$ < 0.637$&$< 0.526$&$ < 0.254$&$< 0.365$&$< 0.225$\\
\hline\hline
            
		\end{tabular}}
	\end{center}
	\caption{Results for \slcdm+$N_{\rm eff}+\Sigma m_\nu$. The constraints on parameters are at $68\%$ CL, while upper bounds are at $95\%$ CL.}
	\label{tab:neffmnu}
\end{table*}

==> Papers/SLCDM/table_neff.tex <==
\begin{table*}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\resizebox{0.9\textwidth}{!}{\begin{tabular}{c c c c  c  c}
  	        \hline
			\textbf{Parameter} & \textbf{Planck}  & \textbf{Planck+Lensing}  & \textbf{Planck+BAO} & \textbf{Planck+Pantheon} & \textbf{Planck+All} \\
			\hline\hline
			$\Omega_{\rm b} h^2$ &$0.02248\pm 0.00026$&$0.02234\pm 0.00024$&$0.02247\pm 0.00019$ & $0.02252\pm 0.00024$ &$0.02241\pm 0.00019$\\
			$\Omega_{\rm c} h^2$ &$0.1170\pm 0.0031$&$0.1161\pm 0.0030$&$0.1166\pm 0.0030$ & $0.1171\pm 0.0031$ &$0.1163\pm 0.0029$\\
			$100\,\theta_{\rm {MC}}$ &$1.04128\pm 0.00046$&$1.04136\pm 0.00046$&$1.04133\pm 0.00046$& $1.04127\pm 0.00046$ &$1.04134\pm 0.00045$\\
			$\tau$   &$0.0512\pm 0.0087$&$0.0503\pm 0.0084$&$0.0515\pm 0.0085$& $0.0514\pm 0.0087$ &$0.0509\pm 0.0086$\\
			$\ln(10^{10}A_{\rm S})$ &$3.148\pm 0.056$&$3.068\pm 0.029$&$3.139\pm 0.043$ & $3.153\pm 0.052$ &$3.075\pm 0.024$\\
			$n_s$ &$0.945\pm 0.016$&$0.950\pm 0.012$&$0.944\pm 0.015$ & $0.0.947\pm 0.016$ &$0.952\pm 0.011$\\
			\hline	
            $H_0$ [km s$^{-1}$ Mpc$^{-1}$] &$67.3\pm 1.7$ &$66.7\pm 1.6$&$67.2\pm 1.2$&$67.6\pm 1.6$&$67.1\pm 1.1$\\
$\sigma_8$& $0.842^{+0.024}_{-0.026}$&$0.810\pm 0.013$&$0.837\pm 0.018$&$0.844\pm 0.023$&$0.812\pm 0.011$\\
$S_8$ &$ 0.855\pm 0.019$&$ 0.827\pm 0.013$&$ 0.849\pm 0.018$&$ 0.853\pm 0.020$&$ 0.824\pm 0.011$\\
$A_{\rm 0} $ &$-0.109\pm 0.050$&$ -0.040^{+0.032}_{-0.027}$&$ -0.101\pm 0.040$&$ -0.113\pm 0.046$&$ -0.045^{+0.030}_{-0.027}$\\
$\epsilon $&$> -0.420$&$> -0.692$&$ >-0.391$&$> -0.388$&$> -0.632$\\
$N_{\rm eff}$&$ 2.93\pm 0.21$&$2.86\pm 0.20$&$2.91\pm 0.18$&$2.96\pm 0.20$&$2.90\pm 0.17$\\
\hline\hline
            
		\end{tabular}}
	\end{center}
	\caption{Results for \slcdm+$N_{\rm eff}$. The constraints on parameters are at $68\%$ CL, while upper bounds are at $95\%$ CL.}
	\label{tab:nnu}
\end{table*}

==> Papers/SLCDM/table_neff_meff.tex <==
\begin{table*}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\resizebox{0.9\textwidth}{!}{\begin{tabular}{c c c c  c  c}
  	        \hline
			\textbf{Parameter} & \textbf{Planck}  & \textbf{Planck+Lensing}  & \textbf{Planck+BAO} & \textbf{Planck+Pantheon} & \textbf{Planck+All} \\
			\hline\hline
  $\Omega_\mathrm{b} h^2$ &$ 0.02271\pm 0.00020$&$ 0.02260\pm 0.00018$&$ 0.02273\pm 0.00020$&$0.02272\pm 0.00019$&$0.02263\pm 0.00016$\\
$\Omega_\mathrm{c} h^2$ & $0.1186^{+0.0037}_{-0.0031}$&$0.1190^{+0.0037}_{-0.0030}$&$0.1180^{+0.0036}_{-0.0031}$&$0.1182^{+0.0038}_{-0.0032}$&$0.1181^{+0.0030}_{-0.0025}$\\
$100\theta_\mathrm{MC}$ & $1.04089\pm 0.00037$&$1.04085\pm 0.00036$&$1.04098\pm 0.00034$&$1.04095\pm 0.00036$&$ 1.04099\pm 0.00032$\\
$\tau_\mathrm{reio}$ &$ 0.0509\pm 0.0086$&$0.0511\pm 0.0087$&$ 0.0514\pm 0.0085$&$0.0515\pm 0.0083$&$0.0520\pm 0.0084$\\
$\log(10^{10} A_\mathrm{s})$ &$ 3.191\pm 0.056$&$3.097\pm 0.033$&$3.187\pm 0.051$&$3.193\pm 0.053$&$3.104\pm 0.031$\\
$n_\mathrm{s}$ &$ 0.954\pm 0.013$&$0.9598\pm 0.0093$&$0.955\pm 0.013$&$0.955\pm 0.013$&$0.9608\pm 0.0089$\\
\hline
$H_0$ [km s$^{-1}$ Mpc$^{-1}$] & $67.97\pm 0.97$&$67.81\pm 0.91$&$68.33^{+0.63}_{-0.78}$&$68.23^{+0.85}_{-0.97}$&$68.23^{+0.57}_{-0.63}$\\
$\sigma_8$ &$ 0.814\pm 0.036$&$0.789^{+0.028}_{-0.024}$&$0.824\pm 0.024$&$ 0.821^{+0.036}_{-0.032}$&$ 0.801^{+0.019}_{-0.017}$\\
$S_8$ &$ 0.834\pm 0.029$& $0.809^{+0.023}_{-0.020}$&$ 0.836\pm 0.023$&$ 0.836^{+0.031}_{-0.027}$&$ 0.812^{+0.019}_{-0.017}$\\
$A_{\rm 0}$ & $-0.140\pm 0.050$&$ -0.056\pm 0.034$&$-0.138\pm 0.046$&$-0.141\pm 0.047$&$-0.063\pm 0.033$\\
$\epsilon$ &$> -0.290$&$> -0.544$&$ > -0.279$&$ > -0.281$&$ > -0.481$\\
$N_{\rm eff}$&$ 3.21^{+0.10}_{-0.14}$&$3.183^{+0.089}_{-0.12}$&$3.176^{+0.088}_{-0.13}$&$3.190^{+0.096}_{-0.14}$&$3.143^{+0.066}_{-0.10}$\\
$m_{\rm eff}$ [eV] &$< 0.893$&$< 0.744$&$< 0.700$&$ < 0.801$&$< 0.571$\\          
\hline\hline
  \end{tabular}}
	\end{center}
	\caption{Results for \slcdm+$N_{\rm eff}+m_{\rm eff}$. The constraints on parameters are at $68\%$ CL, while upper bounds are at $95\%$ CL.}
	\label{tab:nnumeff}
\end{table*}

==> Papers/SLCDM/table_neff_meff_mnu.tex <==
\begin{table*}
	\begin{center}
		\renewcommand{\arraystretch}{1.5}
		\resizebox{0.9\textwidth}{!}{\begin{tabular}{c c c c  c  c}
  	        \hline
			\textbf{Parameter} & \textbf{Planck}  & \textbf{Planck+Lensing}  & \textbf{Planck+BAO} & \textbf{Planck+Pantheon} & \textbf{Planck+All} \\
			\hline\hline
$\Omega_\mathrm{b} h^2$&$0.02268\pm 0.00021$&$0.02255\pm 0.00019$&$0.02273\pm 0.00018$&$0.02273\pm 0.00019$&$0.02263\pm 0.00017$\\
$\Omega_\mathrm{c} h^2$&$ 0.1186^{+0.0038}_{-0.0032}$&$0.1191^{+0.0035}_{-0.0029}$&$0.1177^{+0.0035}_{-0.0030}$&$0.1180^{+0.0038}_{-0.0032}$&$0.1182^{+0.0030}_{-0.0025}$\\
$100\theta_\mathrm{MC} $&$ 1.04083\pm 0.00038$&$1.04081\pm 0.00037$&$1.04100\pm 0.00034$&$1.04094\pm 0.00036$&$1.04098\pm 0.00033$\\
$\tau_\mathrm{reio} $&$0.0507\pm 0.0084$&$0.0507\pm 0.0087$&$0.0514\pm 0.0088$&$0.0515\pm 0.0086$&$0.0515\pm 0.0085$\\
$\log(10^{10} A_\mathrm{s})$&$3.210\pm 0.059$&$3.117^{+0.039}_{-0.044}$&$3.199\pm 0.057$&$3.204\pm 0.056$&$3.109\pm 0.034$\\
$n_\mathrm{s}$&$ 0.952\pm 0.014$&$0.9583\pm 0.0099$&$ 0.955\pm 0.013$&$0.955\pm 0.014$&$0.9612\pm 0.0093$\\
\hline
$H_0$ [km s$^{-1}$ Mpc$^{-1}$] &$66.6^{+1.9}_{-1.7}$&$66.7\pm 1.5$&$68.18\pm 0.73$&$67.8\pm 1.2$&$68.18\pm 0.67$\\
$\sigma_8$&$ 0.787\pm 0.044$&$0.771\pm 0.030$&$0.822\pm 0.025$&$0.813\pm 0.035$&$0.800^{+0.020}_{-0.018}$\\
$S_8$ &$0.828\pm 0.029$&$ 0.809^{+0.022}_{-0.019}$&$ 0.835\pm 0.023$&$ 0.834\pm 0.028$&$ 0.812^{+0.019}_{-0.017}$\\
$A_{\rm 0} $&$-0.156\pm 0.052$&$-0.076\pm 0.041$&$-0.148\pm 0.051$&$ -0.151\pm 0.050$&$ -0.070\pm 0.034$\\
$\epsilon$&$ > -0.264$&$ > -0.457$&$ > -0.277$&$ > -0.268$&$> -0.431$\\
$N_{\rm eff}$ &$3.21^{+0.11}_{-0.15}$&$3.177^{+0.088}_{-0.13}$&$3.168^{+0.083}_{-0.12}$&$3.188^{+0.095}_{-0.14}$&$3.150^{+0.072}_{-0.11}$\\
$\Sigma m_\nu $ [eV]&$< 0.593$&$ < 0.483$&$ < 0.234$&$< 0.335$&$< 0.198$\\
$m_{\rm eff}$ [eV]&$ < 0.909$&$< 0.695$&$< 0.689$&$< 0.790$&$ < 0.550$\\
\hline\hline
		\end{tabular}}
	\end{center}
	\caption{Results for \slcdm+$N_{\rm eff}+m_{\rm eff}+\Sigma m_\nu$. The constraints on parameters are at $68\%$ CL, while upper bounds are at $95\%$ CL.}
	\label{tab:nnumeffmnu}
\end{table*}
